Configuration spaces of an embedding torus and cubical spaces

For a smooth manifold M obtained as an embedding torus, A U Cx[-1,1], we consider the ordered configuration space F_k(M) of k distinct points in M. We show that there is a homotopical cubical resolution of F_k(M) defined from the configuration spaces of A and C. From it, we deduce a universal method for the computation of the pure braid groups of a manifold. We illustrate the method in the case of the Mobius band.

==> GFX/1-k.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Mon Aug 22 10:05:17 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="110" y-min="-10" y-max="0" auto-bounding="true">
%<g>
%<multicurve points="(0,0);(0,0);(10,0);(10,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	 stroke-style="none"
%	 fill-style="none"
%	 />
%<multicurve points="(20,0);(20,0);(30,0);(30,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	 stroke-style="none"
%	 fill-style="none"
%	 />
%<multicurve points="(40,0);(40,0);(50,0);(50,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	 stroke-style="none"
%	 fill-style="none"
%	 />
%<multicurve points="(60,0);(60,0);(70,0);(70,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	 stroke-style="none"
%	 fill-style="none"
%	 />
%<multicurve points="(80,0);(80,0);(90,0);(90,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	 stroke-style="none"
%	 fill-style="none"
%	 />
%<multicurve points="(100,0);(100,0);(110,0);(110,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	 stroke-style="none"
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(0,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(10,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$2$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(110,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$k$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(20,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(40,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$i$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(50,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$j$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(60,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(80,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(100,-10)" text-frame="noframe"
%	 stroke-style="none"
%	 fill-style="none"
%	 >
%$\dots$
%</text>
%</g>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,0)
\psdots[linestyle=none](0,0)
(10,0)
\psdots[linestyle=none](20,0)
(30,0)
\psdots[linestyle=none](40,0)
(50,0)
\psdots[linestyle=none](60,0)
(70,0)
\psdots[linestyle=none](80,0)
(90,0)
\psdots[linestyle=none](100,0)
(110,0)
\rput(0,-10){$1$}
\rput(10,-10){$2$}
\rput(110,-10){$k$}
\rput(20,-10){$\dots$}
\rput(30,-10){$\dots$}
\rput(40,-10){$i$}
\rput(50,-10){$\dots$}
\rput(70,-10){$j$}
\rput(60,-10){$\dots$}
\rput(80,-10){$\dots$}
\rput(90,-10){$\dots$}
\rput(100,-10){$\dots$}
\end{pspicture}


==> GFX/2cellMob-split.1.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Tue Dec 27 02:50:05 CET 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="150" y-min="-2.5" y-max="30" auto-bounding="true">
%<multicurve points="(122.5,15);(122.5,15);(127.5,15);(127.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(132.5,15);(132.5,15);(137.5,15);(137.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(142.5,15);(142.5,15);(147.5,15);(147.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(120,0)" p2="(150,0)" p3="(150,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(127.5,7.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(142.5,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(127.5,15);(127.5,15);(133.75,0);(133.75,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(142.5,15);(142.5,15);(136.25,7.5);(136.25,7.5)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(127.5,15);(127.5,15);(133.75,7.5);(133.75,7.5)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(142.5,15);(142.5,15);(136.25,0);(136.25,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(2.5,15);(2.5,15);(7.5,15);(7.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(12.5,15);(12.5,15);(17.5,15);(17.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(22.5,15);(22.5,15);(27.5,15);(27.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(0,0)" p2="(30,0)" p3="(30,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(7.5,7.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(22.5,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(7.5,15);(7.5,15);(15,0);(15,0)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(22.5,15);(22.5,15);(15,7.5);(15,7.5)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(52.5,15);(52.5,15);(57.5,15);(57.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(42.5,15);(42.5,15);(67.5,15);(67.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(40,0)" p2="(70,0)" p3="(70,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(47.5,7.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(62.5,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(82.5,15);(82.5,15);(87.5,15);(87.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(92.5,15);(92.5,15);(97.5,15);(97.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(102.5,15);(102.5,15);(107.5,15);(107.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(80,0)" p2="(110,0)" p3="(110,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(87.5,7.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(102.5,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(95,7.5);(95,7.5);(87.5,15);(87.5,15)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(95,0);(95,0);(102.5,15);(102.5,15)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(55,7.5);(55,7.5);(55,0);(55,0)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(56.25,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<multicurve points="(58.75,1.25);(63.75,1.88);(65,2.37);(65,3.75);(65,5.13);(60.52,7.5);
%	(55,7.5)"
%	
%	 fill-style="none"
%	 left-arrow="head" arrow-global-scale-width="1.5" />
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(60,3.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<multicurve points="(55,0);(55,0);(55,5);(55,5)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(121.25,-1.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<multicurve points="(136.25,0);(141.25,0.62);(143.75,2.37);(143.75,3.75);(143.75,5.13);(141.78,7.5);
%	(136.25,7.5)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(125,-2.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<multicurve points="(133.75,0);(133.75,0);(133.75,7.5);(133.75,7.5)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(35,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\ast$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(75,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\ast$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(115,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\he$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(150,30)
\psdots[](122.5,15)
(127.5,15)
\psdots[](132.5,15)
(137.5,15)
\psdots[](142.5,15)
(147.5,15)
\pspolygon[](120,0)(150,0)(150,30)(120,30)
\rput[r](127.5,7.5){$x_p$}
\rput[l](142.5,10){$x_q$}
\psline(127.5,15)(133.75,0)
\psline(142.5,15)(136.25,7.5)
\psline(127.5,15)(133.75,7.5)
\psline(142.5,15)(136.25,0)
\psdots[](2.5,15)
(7.5,15)
\psdots[](12.5,15)
(17.5,15)
\psdots[](22.5,15)
(27.5,15)
\pspolygon[](0,0)(30,0)(30,30)(0,30)
\rput[r](7.5,7.5){$x_p$}
\rput[l](22.5,10){$x_q$}
\psline[arrowscale=1.5 1.5]{->}(7.5,15)(15,0)
\psline[arrowscale=1.5 1.5]{->}(22.5,15)(15,7.5)
\psdots[](52.5,15)
(57.5,15)
\psdots[](42.5,15)
(67.5,15)
\pspolygon[](40,0)(70,0)(70,30)(40,30)
\rput[r](47.5,7.5){$x_p$}
\rput[l](62.5,10){$x_q$}
\psdots[](82.5,15)
(87.5,15)
\psdots[](92.5,15)
(97.5,15)
\psdots[](102.5,15)
(107.5,15)
\pspolygon[](80,0)(110,0)(110,30)(80,30)
\rput[r](87.5,7.5){$x_p$}
\rput[l](102.5,10){$x_q$}
\psline[arrowscale=1.5 1.5]{->}(95,7.5)(87.5,15)
\psline[arrowscale=1.5 1.5]{->}(95,0)(102.5,15)
\psdots[](55,7.5)
(55,0)
\rput(56.25,5){}
\pscustom[arrowscale=1.5 1]{\psbezier{<-}(58.75,1.25)(63.75,1.88)(65,2.37)(65,3.75)
\psbezier{-}(65,3.75)(65,5.13)(60.52,7.5)(55,7.5)
}
\rput[l](60,3.75){}
\psline[arrowscale=1.5 1]{->}(55,0)(55,5)
\rput(121.25,-1.25){}
\pscustom[]{\psbezier(136.25,0)(141.25,0.62)(143.75,2.37)(143.75,3.75)
\psbezier(143.75,3.75)(143.75,5.13)(141.78,7.5)(136.25,7.5)
}
\rput[l](125,-2.5){}
\psline(133.75,0)(133.75,7.5)
\rput(35,15){$\ast$}
\rput(75,15){$\ast$}
\rput(115,15){$\he$}
\end{pspicture}


==> GFX/E3-final.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Wed Oct 12 16:25:53 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="75" y-min="0" y-max="50" auto-bounding="true">
%<multicurve points="(20,20);(20,20);(40,12.5);(40,12.5)"
%	 stroke-width="0.5" stroke-color="#ff0000"
%	 fill-style="none"
%	 right-arrow="head" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(45,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$E^2(A)$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(75,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\FF_2(A\times\RR)$
%</text>
%<multicurve points="(52.5,10);(52.5,10);(65,10);(65,10)"
%	 stroke-width="0.5" stroke-color="#ff0000"
%	 fill-style="none"
%	 right-arrow="head" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(75,40)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\FF_3(A\times\RR)$
%</text>
%<multicurve points="(75,37.5);(75,37.5);(75,12.5);(75,12.5)"
%	 stroke-width="0.5" stroke-color="#ff0000"
%	 fill-style="none"
%	 right-arrow="head" stroke-overstrike="true" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(45,40)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$E^3(A)$
%</text>
%<multicurve points="(52.5,40);(52.5,40);(65,40);(65,40)"
%	 stroke-width="0.5" stroke-color="#ff0000"
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(45,37.5);(45,37.5);(45,12.5);(45,12.5)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" stroke-overstrike="true" stroke-overstrike-width="0.9" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(17.5,20)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$A^2$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(5,10)" text-frame="noframe"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 >
%$\FF_2(A)$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(32.5,0)" text-frame="noframe"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 >
%$A^2$
%</text>
%<multicurve points="(35,0);(35,0);(42.5,7.5);(42.5,7.5)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(7.5,12.5);(7.5,12.5);(15,20);(15,20)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(10,7.5);(10,7.5);(30,0);(30,0)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(32.5,30)" text-frame="noframe"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 >
%$E^3_3$
%</text>
%<multicurve points="(35,30);(35,30);(42.5,37.5);(42.5,37.5)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(7.5,42.5);(7.5,42.5);(15,50);(15,50)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(17.5,50)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$E^3_1$
%</text>
%<multicurve points="(20,50);(20,50);(40,42.5);(40,42.5)"
%	 stroke-width="0.5" stroke-color="#ff0000"
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(17.5,47.5);(17.5,47.5);(17.5,22.5);(17.5,22.5)"
%	 stroke-width="0.5" stroke-color="#ff0000"
%	 fill-style="none"
%	 right-arrow="head" stroke-overstrike="true" stroke-overstrike-width="0.9" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(5,40)" text-frame="noframe"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 >
%$E^3_2$
%</text>
%<multicurve points="(10,37.5);(10,37.5);(30,30);(30,30)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" stroke-overstrike="true" stroke-overstrike-width="0.9" />
%<multicurve points="(5,37.5);(5,37.5);(5,12.5);(5,12.5)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" stroke-overstrike="true" stroke-overstrike-width="0.9" />
%<multicurve points="(32.5,27.5);(32.5,27.5);(32.5,2.5);(32.5,2.5)"
%	 stroke-color="#3c3c3c"
%	 fill-style="none"
%	 right-arrow="head" stroke-overstrike="true" stroke-overstrike-width="0.9" />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(75,50)
\psline[linewidth=0.5,linecolor=red]{->}(20,20)(40,12.5)
\rput(45,10){$E^2(A)$}
\rput(75,10){$\FF_2(A\times\RR)$}
\psline[linewidth=0.5,linecolor=red]{->}(52.5,10)(65,10)
\rput(75,40){$\FF_3(A\times\RR)$}
\psline[linewidth=0.5,linecolor=red,border=0.3]{->}(75,37.5)(75,12.5)
\rput(45,40){$E^3(A)$}
\psline[linewidth=0.5,linecolor=red]{->}(52.5,40)(65,40)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour,border=0.9]{->}(45,37.5)(45,12.5)
\rput(17.5,20){$A^2$}
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\rput(5,10){$\FF_2(A)$}
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\rput(32.5,0){$A^2$}
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour]{->}(35,0)(42.5,7.5)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour]{->}(7.5,12.5)(15,20)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour]{->}(10,7.5)(30,0)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\rput(32.5,30){$E^3_3$}
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour]{->}(35,30)(42.5,37.5)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour]{->}(7.5,42.5)(15,50)
\rput(17.5,50){$E^3_1$}
\psline[linewidth=0.5,linecolor=red]{->}(20,50)(40,42.5)
\psline[linewidth=0.5,linecolor=red,border=0.9]{->}(17.5,47.5)(17.5,22.5)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\rput(5,40){$E^3_2$}
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour,border=0.9]{->}(10,37.5)(30,30)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour,border=0.9]{->}(5,37.5)(5,12.5)
\newrgbcolor{userLineColour}{0.24 0.24 0.24}
\psline[linecolor=userLineColour,border=0.9]{->}(32.5,27.5)(32.5,2.5)
\end{pspicture}


==> GFX/Exemple-FF2.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Thu Oct 06 12:28:27 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="65" y-min="-0.46" y-max="49.8" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(15,37.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(15,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$-q$
%</text>
%<circle p1="(60,25)" p2="(40,0)" p3="(15,10)" closure="open"
%	
%	 fill-style="none"
%	 />
%<circle p1="(52.5,25)" p2="(43.63,7.18)" p3="(15,10)" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(47.5,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(65,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_2$
%</text>
%<circle p1="(15,40)" p2="(39.08,44.58)" p3="(52.5,25)" closure="open"
%	
%	 fill-style="none"
%	 left-arrow="head" arrow-global-scale-width="1.5" />
%<circle p1="(15,40)" p2="(39.77,49.32)" p3="(60,25)" closure="open"
%	
%	 fill-style="none"
%	 left-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<circle p1="(0,25)" p2="(15,40)" p3="(30,25)" closure="open"
%	
%	 fill-style="none"
%	 left-arrow="head" right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<circle p1="(0,25)" p2="(15,10)" p3="(30,25)" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(2.5,32.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(22.5,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$y$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(5,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(65,49.8)
\rput(15,37.5){$q$}
\rput(15,12.5){$-q$}
\rput{0}(35.23,24.32){\parametricplot[arrows=-]{-144.71}{1.58}{ t cos 24.78 mul t sin 24.78 mul }}
\rput{0}(30.89,24.64){\parametricplot[arrows=-]{-137.35}{0.95}{ t cos 21.61 mul t sin 21.61 mul }}
\rput(47.5,25){$z_1$}
\rput(65,25){$z_2$}
\rput{0}(30.47,24.29){\parametricplot[arrowscale=1.5 1,arrows=<-]{1.84}{134.56}{ t cos 22.04 mul t sin 22.04 mul }}
\rput{0}(34.9,24.69){\parametricplot[arrowscale=1.5 1,arrows=>-]{0.7}{142.43}{ t cos 25.1 mul t sin 25.1 mul }}
\rput{0}(15,25){\parametricplot[arrowscale=1.5 1,arrows=<-<]{0}{180}{ t cos 15 mul t sin 15 mul }}
\rput{0}(15,25){\parametricplot[arrows=-]{180}{360}{ t cos 15 mul t sin 15 mul }}
\rput(2.5,32.5){}
\rput(22.5,25){$y$}
\rput(5,25){$x$}
\end{pspicture}


==> GFX/Hocolim-exempleVogt.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Thu Sep 22 11:25:39 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-12.5" x-max="35" y-min="2.5" y-max="35" auto-bounding="true">
%<text text-vert-align="top" text-hor-align="right" anchor-point="(6.25,6.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\bar i_2\circ \bar f_1\circ\bar f_0$
%</text>
%<text text-vert-align="top" text-hor-align="left" anchor-point="(33.75,6.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\bar i_2\circ \bar  f_2$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(20,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\bar i_2\circ H$
%</text>
%<text text-vert-align="top" text-hor-align="right" anchor-point="(-12.5,2.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<text text-vert-align="baseline" text-hor-align="right" anchor-point="(6.25,33.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\bar i_1\circ\bar f_0$
%</text>
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(5,20)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$L\circ\bar f_0$
%</text>
%<text text-vert-align="baseline" text-hor-align="left" anchor-point="(33.75,33.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\bar i_0$
%</text>
%<text text-vert-align="baseline" text-hor-align="center-h" anchor-point="(20,35)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$K$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(35,20)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$M$
%</text>
%<multicurve points="(7.5,32.5);(7.5,32.5);(32.5,32.5);(32.5,32.5)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(32.5,32.5);(32.5,32.5);(32.5,7.5);(32.5,7.5)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(32.5,7.5);(32.5,7.5);(7.5,7.5);(7.5,7.5)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(7.5,7.5);(7.5,7.5);(7.5,32.5);(7.5,32.5)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,35)
\rput[tr](6.25,6.25){$\bar i_2\circ \bar f_1\circ\bar f_0$}
\rput[tl](33.75,6.25){$\bar i_2\circ \bar  f_2$}
\rput[t](20,5){$\bar i_2\circ H$}
\rput[tr](-12.5,2.5){}
\rput[Br](6.25,33.75){$\bar i_1\circ\bar f_0$}
\rput[r](5,20){$L\circ\bar f_0$}
\rput[Bl](33.75,33.75){$\bar i_0$}
\rput[B](20,35){$K$}
\rput[l](35,20){$M$}
\psline(7.5,32.5)(32.5,32.5)
\psdots[](7.5,32.5)
(32.5,32.5)
\psline(32.5,32.5)(32.5,7.5)
\psdots[](32.5,32.5)
(32.5,7.5)
\psline(32.5,7.5)(7.5,7.5)
\psdots[](32.5,7.5)
(7.5,7.5)
\psline(7.5,7.5)(7.5,32.5)
\psdots[](7.5,7.5)
(7.5,32.5)
\end{pspicture}


==> GFX/Massey.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Tue Sep 20 13:54:46 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10.13" x-max="56.51" y-min="0" y-max="41.25" auto-bounding="true">
%<ellipse p1="(10.13,40)" p2="(50.13,40)" p3="(50.13,0)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30.07,17.57)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<multicurve points="(46.58,31.25);(46.58,31.25);(30,20);(30,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(34.93,34.93)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_3$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(47.5,34.01)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_2$
%</text>
%<ellipse p1="(36.51,41.25)" p2="(56.51,41.25)" p3="(56.51,21.25)" angle-start="0" angle-end="0" closure="open"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 stroke-overstrike="true" stroke-overstrike-width="1" />
%<ellipse p1="(20,30)" p2="(40,30)" p3="(40,10)" angle-start="0" angle-end="0" closure="open"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(36.97,34.21);(36.97,34.21);(30,20);(30,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(56.51,41.25)
\rput{0}(30.13,20){\psellipse[](0,0)(20,-20)}
\rput(30.07,17.57){$q_1$}
\psdots[](46.58,31.25)
(30,20)
\rput[r](34.93,34.93){$x_3$}
\rput[l](47.5,34.01){$x_2$}
\rput{0}(46.51,31.25){\psellipse[linestyle=dashed,dash=1 1,border=1](0,0)(10,-10)}
\rput{0}(30,20){\psellipse[linestyle=dashed,dash=1 1](0,0)(10,-10)}
\psdots[](36.97,34.21)
(30,20)
\end{pspicture}


==> GFX/Mobius-X1b.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Tue Jan 10 14:17:01 CET 2006
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="0" y-max="30" auto-bounding="true">
%<multicurve points="(5,15);(5,15);(15,15);(15,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(27.5,15);(27.5,15);(31.25,30);(31.25,30)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(31.25,30);(31.25,30);(40,15);(40,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(0,0)" p2="(65,0)" p3="(65,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(5,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<text text-vert-align="top" text-hor-align="right" anchor-point="(30,28.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_r$
%</text>
%<text text-vert-align="bottom" text-hor-align="center-h" anchor-point="(42.5,21.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_{j+1}$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(15,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_i$
%</text>
%<multicurve points="(26.25,15);(26.25,15);(20,15);(20,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(10,15);(10,15);(6.25,15);(6.25,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(31.25,30);(31.25,30);(35,15);(35,15)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<ellipse p1="(11.25,25)" p2="(18.75,25)" p3="(18.75,5)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(51.25,15);(51.25,15);(46.25,15);(46.25,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(46.25,15);(46.25,17.5);(46.25,20);(43.75,20);(41.25,20);(26.25,20);
%	(23.75,20);(21.25,20);(18.75,20);(18.75,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(45,15);(45,15);(41.25,15);(41.25,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(60,15);(60,15);(51.25,15);(51.25,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(58.75,15);(58.75,15);(55,15);(55,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(80,15);(80,15);(90,15);(90,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(102.5,15);(102.5,15);(106.25,30);(106.25,30)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(106.25,30);(106.25,30);(115,15);(115,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(75,0)" p2="(140,0)" p3="(140,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(80,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<text text-vert-align="top" text-hor-align="right" anchor-point="(105,28.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_r$
%</text>
%<text text-vert-align="bottom" text-hor-align="center-h" anchor-point="(118.75,21.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_{j+1}$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(90,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_i$
%</text>
%<multicurve points="(101.25,15);(101.25,15);(95,15);(95,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(85,15);(85,15);(81.25,15);(81.25,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(106.25,30);(106.25,30);(110,15);(110,15)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<ellipse p1="(86.25,25)" p2="(93.75,25)" p3="(93.75,5)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(126.25,15);(126.25,15);(121.25,15);(121.25,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(121.25,15);(121.25,17.5);(121.25,20);(118.75,20);(116.25,20);(112.5,20);
%	(112.5,15);(112.5,10);(106.25,10);(106.25,15);(106.25,20);(101.25,20);
%	(98.75,20);(96.25,20);(93.75,20);(93.75,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(120,15);(120,15);(116.25,15);(116.25,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(135,15);(135,15);(126.25,15);(126.25,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(133.75,15);(133.75,15);(130,15);(130,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,30)
\psdots[](5,15)
(15,15)
\psdots[](27.5,15)
(31.25,30)
\psdots[](31.25,30)
(40,15)
\pspolygon[](0,0)(65,0)(65,30)(0,30)
\rput[t](5,12.5){$q_1$}
\rput[tr](30,28.75){$x_r$}
\rput[b](42.5,21.25){$x_{j+1}$}
\rput[t](15,12.5){$q_i$}
\psline[linestyle=dotted](26.25,15)(20,15)
\psline[linestyle=dotted](10,15)(6.25,15)
\psline[linestyle=dashed,dash=1 1](31.25,30)(35,15)
\rput{90}(15,15){\psellipse[](0,0)(10,-3.75)}
\psline(51.25,15)(46.25,15)
\pscustom[]{\psbezier(46.25,15)(46.25,17.5)(46.25,20)(43.75,20)
\psbezier(43.75,20)(41.25,20)(26.25,20)(23.75,20)
\psbezier(23.75,20)(21.25,20)(18.75,20)(18.75,15)
}
\psline[linestyle=dotted](45,15)(41.25,15)
\psdots[](60,15)
(51.25,15)
\psline[linestyle=dotted](58.75,15)(55,15)
\psdots[](80,15)
(90,15)
\psdots[](102.5,15)
(106.25,30)
\psdots[](106.25,30)
(115,15)
\pspolygon[](75,0)(140,0)(140,30)(75,30)
\rput[t](80,12.5){$q_1$}
\rput[tr](105,28.75){$x_r$}
\rput[b](118.75,21.25){$x_{j+1}$}
\rput[t](90,12.5){$q_i$}
\psline[linestyle=dotted](101.25,15)(95,15)
\psline[linestyle=dotted](85,15)(81.25,15)
\psline[linestyle=dashed,dash=1 1](106.25,30)(110,15)
\rput{90}(90,15){\psellipse[](0,0)(10,-3.75)}
\psline(126.25,15)(121.25,15)
\pscustom[]{\psbezier(121.25,15)(121.25,17.5)(121.25,20)(118.75,20)
\psbezier(118.75,20)(116.25,20)(112.5,20)(112.5,15)
\psbezier(112.5,15)(112.5,10)(106.25,10)(106.25,15)
\psbezier(106.25,15)(106.25,20)(101.25,20)(98.75,20)
\psbezier(98.75,20)(96.25,20)(93.75,20)(93.75,15)
}
\psline[linestyle=dotted](120,15)(116.25,15)
\psdots[](135,15)
(126.25,15)
\psline[linestyle=dotted](133.75,15)(130,15)
\end{pspicture}


==> GFX/RP2-rel1.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Mon Sep 26 13:29:51 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="-10" y-max="65" auto-bounding="true">
%<multicurve points="(30,40);(30,40);(30,10);(30,10)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(60,40);(60,40);(60,10);(60,10)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,25);(40,25);(50,25);(50,25)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(32.5,38.75);(32.5,38.75);(32.5,20);(32.5,20)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(32.5,10);(32.5,-10);(7.5,15);(5,40);(2.5,65);(57.5,58.75);
%	(57.5,40)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(57.5,40);(57.5,40);(57.5,25);(57.5,25)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(57.5,25);(57.5,25);(57.5,11.25);(57.5,11.25)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(57.5,10);(57.5,-1.25);(35,0);(17.5,0);(0,0);(7.5,20);
%	(10,30);(12.5,40);(15,50);(22.5,50);(30,50);(32.5,45);
%	(32.5,37.5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(32.5,20);(32.5,20);(32.5,10);(32.5,10)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,25);(50,35);(45,35);(40,35);(35,35);(32.5,30);
%	(32.5,25)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(40,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(50,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_2$
%</text>
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(2.5,27.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\sigma_1$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(60,65)
\psline(30,40)(30,10)
\psline(60,40)(60,10)
\psdots[](40,25)
(50,25)
\psline{->}(32.5,38.75)(32.5,20)
\pscustom[linestyle=dashed,dash=1 1]{\psbezier(32.5,10)(32.5,-10)(7.5,15)(5,40)
\psbezier(5,40)(2.5,65)(57.5,58.75)(57.5,40)
}
\psline{->}(57.5,40)(57.5,25)
\psline(57.5,25)(57.5,11.25)
\pscustom[linestyle=dashed,dash=1 1]{\psbezier(57.5,10)(57.5,-1.25)(35,0)(17.5,0)
\psbezier(17.5,0)(0,0)(7.5,20)(10,30)
\psbezier(10,30)(12.5,40)(15,50)(22.5,50)
\psbezier(22.5,50)(30,50)(32.5,45)(32.5,37.5)
}
\psline(32.5,20)(32.5,10)
\pscustom[]{\psbezier(50,25)(50,35)(45,35)(40,35)
\psbezier(40,35)(35,35)(32.5,30)(32.5,25)
}
\rput[t](40,22.5){$q_1$}
\rput[t](50,22.5){$x_2$}
\rput[r](2.5,27.5){$\sigma_1$}
\end{pspicture}


==> GFX/YB-Phi.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sun Sep 18 19:44:51 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15" x-max="45" y-min="-7.5" y-max="22.5" auto-bounding="true">
%<ellipse p1="(15,22.5)" p2="(45,22.5)" p3="(45,-7.5)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(22.5,15)" p2="(37.5,15)" p3="(37.5,0)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30.53,5.39)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<multicurve points="(40,18.75);(40,18.75);(30,7.5);(30,7.5)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(26.25,13.75);(26.25,13.75);(30,7.5);(30,7.5)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(23.68,15.66)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_3$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(43.95,20.13)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_2$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(45,22.5)
\rput{0}(30,7.5){\psellipse[](0,0)(15,-15)}
\rput{0}(30,7.5){\psellipse[](0,0)(7.5,-7.5)}
\rput(30.53,5.39){$q_1$}
\psdots[](40,18.75)
(30,7.5)
\psdots[](26.25,13.75)
(30,7.5)
\rput(23.68,15.66){$x_3$}
\rput(43.95,20.13){$x_2$}
\end{pspicture}


==> GFX/YB-Psi.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sun Sep 18 19:43:54 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15.26" x-max="51.84" y-min="-7.37" y-max="26.38" auto-bounding="true">
%<ellipse p1="(15.26,22.63)" p2="(45.26,22.63)" p3="(45.26,-7.37)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(32.76,26.38)" p2="(47.76,26.38)" p3="(47.76,11.38)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30.33,4.8)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<multicurve points="(40.26,18.88);(40.26,18.88);(30.26,7.63);(30.26,7.63)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(47.76,17.63);(47.76,17.63);(30.26,7.63);(30.26,7.63)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(51.84,17.96)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_3$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(41.18,21.58)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_2$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(51.84,26.38)
\rput{0}(30.26,7.63){\psellipse[](0,0)(15,-15)}
\rput{0}(40.26,18.88){\psellipse[](0,0)(7.5,-7.5)}
\rput(30.33,4.8){$q_1$}
\psdots[](40.26,18.88)
(30.26,7.63)
\psdots[](47.76,17.63)
(30.26,7.63)
\rput(51.84,17.96){$x_3$}
\rput(41.18,21.58){$x_2$}
\end{pspicture}


==> GFX/YB-Upsilon.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sun Sep 18 19:44:27 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15" x-max="74.38" y-min="-6.25" y-max="23.75" auto-bounding="true">
%<ellipse p1="(15,23.75)" p2="(45,23.75)" p3="(45,-6.25)" angle-start="0" angle-end="360" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(57.5,16.25)" p2="(72.5,16.25)" p3="(72.5,1.25)" angle-start="0" angle-end="360" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30,6.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_1$
%</text>
%<multicurve points="(40,20);(40,20);(30,8.75);(30,8.75)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(70.62,13.75);(70.62,13.75);(65,8.75);(65,8.75)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(74.38,15.62)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_4$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(43.75,20.62)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_2$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(65,6.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$q_3$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(74.38,23.75)
\rput{0}(30,8.75){\psellipse[](0,0)(15,-15)}
\rput{0}(65,8.75){\psellipse[](0,0)(7.5,-7.5)}
\rput(30,6.25){$q_1$}
\psdots[](40,20)
(30,8.75)
\psdots[](70.62,13.75)
(65,8.75)
\rput(74.38,15.62){$x_4$}
\rput(43.75,20.62){$x_2$}
\rput(65,6.25){$q_3$}
\end{pspicture}


==> GFX/cubiq-2cell-simple.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Thu Sep 15 02:41:36 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="12.5" x-max="50" y-min="7.5" y-max="47.5" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="right" anchor-point="(12.5,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^-(p)\times I$
%</text>
%<multicurve points="(15,40);(15,40);(45,40);(45,40)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(45,40);(45,40);(45,10);(45,10)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(45,25);(45,25);(45,10);(45,10)"
%	
%	 fill-style="none"
%	 left-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<multicurve points="(45,10);(45,10);(15,10);(15,10)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(30,10);(30,10);(15,10);(15,10)"
%	
%	 fill-style="none"
%	 left-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<multicurve points="(15,10);(15,10);(15,25);(15,25)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<multicurve points="(15,10);(15,10);(15,40);(15,40)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="true"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(15,40);(15,40);(30,40);(30,40)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(30,7.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_2^-(p)\times I$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(30,47.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_2^+(p)\times I$
%</text>
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(50,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^+(p)\times I$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(50,47.5)
\rput[r](12.5,25){$d_1^-(p)\times I$}
\psline(15,40)(45,40)
\psdots[](15,40)
(45,40)
\psline(45,40)(45,10)
\psdots[](45,40)
(45,10)
\psline[arrowscale=2 2]{<-}(45,25)(45,10)
\psline(45,10)(15,10)
\psdots[](45,10)
(15,10)
\psline[arrowscale=2 2]{<-}(30,10)(15,10)
\psline[arrowscale=2 2]{->}(15,10)(15,25)
\psline(15,10)(15,40)
\psdots[](15,10)
(15,40)
\psline[arrowscale=2 2]{->}(15,40)(30,40)
\rput[t](30,7.5){$d_2^-(p)\times I$}
\rput[t](30,47.5){$d_2^+(p)\times I$}
\rput[l](50,22.5){$d_1^+(p)\times I$}
\end{pspicture}


==> GFX/cubiq-realisation-2cell.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sat Sep 24 10:08:30 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="120" y-min="-5" y-max="115" auto-bounding="true">
%<multicurve points="(60,110);(60,110);(60,70);(60,70)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(70,60);(70,60);(110,60);(110,60)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(110,60);(110,60);(110,100);(110,100)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(60,110);(60,110);(100,110);(100,110)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(100,110);(100,110);(60,70);(60,70)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(110,100);(110,100);(70,60);(70,60)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,50);(0,50);(0,10);(0,10)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(10,0);(10,0);(50,0);(50,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,0);(50,0);(50,40);(50,40)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,50);(0,50);(40,50);(40,50)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,50);(40,50);(0,10);(0,10)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,40);(50,40);(10,0);(10,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(60,40);(60,40);(100,0);(100,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(100,0);(100,0);(60,0);(60,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(60,40);(60,40);(60,0);(60,0)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(70,50);(70,50);(110,50);(110,50)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(110,50);(110,50);(110,10);(110,10)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(110,10);(110,10);(70,50);(70,50)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,100);(0,100);(40,60);(40,60)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,60);(40,60);(0,60);(0,60)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,100);(0,100);(0,60);(0,60)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(10,110);(10,110);(50,110);(50,110)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,110);(50,110);(50,70);(50,70)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,70);(50,70);(10,110);(10,110)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(55,90)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_2^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(55,20)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_2^-$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(20,55)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^-$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,55)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,80)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(80,115)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(80,-5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(-10,80)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30,-5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^-$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(30,115)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^-$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(-10,30)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^-$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,30)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_1^-$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(85,85)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_{1,2}^{++}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(85,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_{1,2}^{+-}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(25,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_{1,2}^{--}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(25,85)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$d_{1,2}^{-+}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,100)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$F$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(100,70)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$G$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(100,40)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$H$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$I$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(40,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$J$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(10,37.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$K$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(10,70)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$L$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(40,100)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$M$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(55,55)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(120,115)
\psline(60,110)(60,70)
\psline(70,60)(110,60)
\psline(110,60)(110,100)
\psline(60,110)(100,110)
\psline(100,110)(60,70)
\psline(110,100)(70,60)
\psline(0,50)(0,10)
\psline(10,0)(50,0)
\psline(50,0)(50,40)
\psline(0,50)(40,50)
\psline(40,50)(0,10)
\psline(50,40)(10,0)
\psline(60,40)(100,0)
\psline(100,0)(60,0)
\psline(60,40)(60,0)
\psline(70,50)(110,50)
\psline(110,50)(110,10)
\psline(110,10)(70,50)
\psline(0,100)(40,60)
\psline(40,60)(0,60)
\psline(0,100)(0,60)
\psline(10,110)(50,110)
\psline(50,110)(50,70)
\psline(50,70)(10,110)
\rput(55,90){$d_2^+$}
\rput(55,20){$d_2^-$}
\rput(20,55){$d_1^-$}
\rput(90,55){$d_1^+$}
\rput(120,80){$d_1^+$}
\rput(80,115){$d_1^+$}
\rput(80,-5){$d_1^+$}
\rput(-10,80){$d_1^+$}
\rput(30,-5){$d_1^-$}
\rput(30,115){$d_1^-$}
\rput(-10,30){$d_1^-$}
\rput(120,30){$d_1^-$}
\rput(85,85){$d_{1,2}^{++}$}
\rput(85,25){$d_{1,2}^{+-}$}
\rput(25,25){$d_{1,2}^{--}$}
\rput(25,85){$d_{1,2}^{-+}$}
\rput(70,100){$F$}
\rput(100,70){$G$}
\rput(100,40){$H$}
\rput(70,10){$I$}
\rput(40,10){$J$}
\rput(10,37.5){$K$}
\rput(10,70){$L$}
\rput(40,100){$M$}
\rput(55,55){$x$}
\end{pspicture}


==> GFX/schema-4pos.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Mon Aug 29 15:46:48 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="0" y-max="100" auto-bounding="true">
%<multicurve points="(5,20);(5,20);(15,20);(15,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(25,20);(25,20);(35,20);(35,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(45,20);(45,20);(55,20);(55,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(0,0)" p2="(60,0)" p3="(60,40)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(15,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(45,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(15,20);(15,20);(30,0);(30,0)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(45,20);(45,20);(30,5);(30,5)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(85,20);(85,20);(95,20);(95,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(105,20);(105,20);(115,20);(115,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(125,20);(125,20);(135,20);(135,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(80,0)" p2="(140,0)" p3="(140,40)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(95,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(125,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(95,20);(95,20);(110,35);(110,35)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(125,20);(125,20);(110,0);(110,0)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(5,80);(5,80);(15,80);(15,80)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(25,80);(25,80);(35,80);(35,80)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(45,80);(45,80);(55,80);(55,80)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(0,60)" p2="(60,60)" p3="(60,100)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(15,75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(45,75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(15,80);(15,80);(30,65);(30,65)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(45,80);(45,80);(30,100);(30,100)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(85,80);(85,80);(95,80);(95,80)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(105,80);(105,80);(115,80);(115,80)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(125,80);(125,80);(135,80);(135,80)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<parallelogram p1="(80,60)" p2="(140,60)" p3="(140,100)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(95,75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_p$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(125,75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_q$
%</text>
%<multicurve points="(95,80);(95,80);(110,100);(110,100)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<multicurve points="(125,80);(125,80);(110,95);(110,95)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" arrow-global-scale-length="1.5" />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(20,45)" text-frame="circle"
%	
%	 fill-style="none"
%	 >
%$\alpha_1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(40,55)" text-frame="circle"
%	
%	 fill-style="none"
%	 >
%$\alpha_2$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(100,45)" text-frame="circle"
%	
%	 fill-style="none"
%	 >
%$\alpha_4$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,55)" text-frame="circle"
%	
%	 fill-style="none"
%	 >
%$\alpha_3$
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,100)
\psdots[](5,20)
(15,20)
\psdots[](25,20)
(35,20)
\psdots[](45,20)
(55,20)
\pspolygon[](0,0)(60,0)(60,40)(0,40)
\rput(15,15){$x_p$}
\rput(45,15){$x_q$}
\psline[arrowscale=1.5 1.5]{->}(15,20)(30,0)
\psline[arrowscale=1.5 1.5]{->}(45,20)(30,5)
\psdots[](85,20)
(95,20)
\psdots[](105,20)
(115,20)
\psdots[](125,20)
(135,20)
\pspolygon[](80,0)(140,0)(140,40)(80,40)
\rput(95,15){$x_p$}
\rput(125,15){$x_q$}
\psline[arrowscale=1.5 1.5]{->}(95,20)(110,35)
\psline[arrowscale=1.5 1.5]{->}(125,20)(110,0)
\psdots[](5,80)
(15,80)
\psdots[](25,80)
(35,80)
\psdots[](45,80)
(55,80)
\pspolygon[](0,60)(60,60)(60,100)(0,100)
\rput(15,75){$x_p$}
\rput(45,75){$x_q$}
\psline[arrowscale=1.5 1.5]{->}(15,80)(30,65)
\psline[arrowscale=1.5 1.5]{->}(45,80)(30,100)
\psdots[](85,80)
(95,80)
\psdots[](105,80)
(115,80)
\psdots[](125,80)
(135,80)
\pspolygon[](80,60)(140,60)(140,100)(80,100)
\rput(95,75){$x_p$}
\rput(125,75){$x_q$}
\psline[arrowscale=1.5 1.5]{->}(95,80)(110,100)
\psline[arrowscale=1.5 1.5]{->}(125,80)(110,95)
\rput(20,45){\pscirclebox[]{$\alpha_1$}}
\rput(40,55){\pscirclebox[]{$\alpha_2$}}
\rput(100,45){\pscirclebox[]{$\alpha_4$}}
\rput(120,55){\pscirclebox[]{$\alpha_3$}}
\end{pspicture}


==> GFX/tore-X2a.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sat Sep 03 14:54:04 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="145" y-min="3.75" y-max="35" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2t-1$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(80,3.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\rho_{j,t}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2t$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(30,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<ellipse p1="(115,20)" p2="(125,20)" p3="(125,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(65,20)" p2="(75,20)" p3="(75,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(85,20)" p2="(95,20)" p3="(95,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,15);(0,15);(10,15);(10,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,15);(20,15);(30,15);(30,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,15);(40,15);(50,15);(50,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(57.5,15);(57.5,15);(62.5,15);(62.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(30,15);(30,22.5);(28.75,25);(37.5,25);(46.25,25);(62.5,25);
%	(70,25)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(70,25);(77.5,25);(78.75,25);(85,25);(91.25,25);(95,18.75);
%	(95,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(95,15);(95,5);(90,5);(80,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(65,15);(65,5);(70,5);(80,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(30,15);(31.25,22.5);(32.5,22.5);(37.5,22.5);(42.5,22.5);(45,22.5);
%	(50,22.5)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,22.5);(57.5,22.5);(55,22.5);(60,22.5);(65,22.5);(65,18.75);
%	(65,15)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(82.5,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<ellipse p1="(135,20)" p2="(145,20)" p3="(145,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s-1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(140,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s$
%</text>
%<multicurve points="(90,35);(97.5,35);(117.5,35);(130,35);(142.5,35);(145,18.75);
%	(145,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(145,15);(145,5);(140,5);(130,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(115,15);(115,5);(120,5);(130,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(131.25,3.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\rho_{i,s}$
%</text>
%<multicurve points="(10,15);(10,22.5);(16.25,35);(25,35);(33.75,35);(85,35);
%	(90,35)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(72.5,30);(78.75,30);(100,30);(107.5,30);(115,30);(115,18.75);
%	(115,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(10,15);(11.25,22.5);(17.5,30);(25,30);(32.5,30);(68.75,30);
%	(72.5,30)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(10,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_i$
%</text>
%<multicurve points="(97.5,15);(97.5,15);(112.5,15);(112.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(145,35)
\rput(70,15){$\scriptstyle 2t-1$}
\rput[t](80,3.75){$\rho_{j,t}$}
\rput(90,15){$\scriptstyle 2t$}
\rput[t](30,12.5){$x_j$}
\rput{0}(120,15){\psellipse[](0,0)(5,-5)}
\rput{0}(70,15){\psellipse[](0,0)(5,-5)}
\rput{0}(90,15){\psellipse[](0,0)(5,-5)}
\psdots[](0,15)
(10,15)
\psdots[](20,15)
(30,15)
\psdots[](40,15)
(50,15)
\psline[linestyle=dotted](57.5,15)(62.5,15)
\pscustom[]{\psbezier(30,15)(30,22.5)(28.75,25)(37.5,25)
\psbezier(37.5,25)(46.25,25)(62.5,25)(70,25)
}
\pscustom[]{\psbezier(70,25)(77.5,25)(78.75,25)(85,25)
\psbezier(85,25)(91.25,25)(95,18.75)(95,15)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(95,15)(95,5)(90,5)(80,5)
\psbezier[linestyle=dashed,dash=1 1](65,15)(65,5)(70,5)(80,5)
\pscustom[]{\psbezier(30,15)(31.25,22.5)(32.5,22.5)(37.5,22.5)
\psbezier(37.5,22.5)(42.5,22.5)(45,22.5)(50,22.5)
}
\pscustom[]{\psbezier(50,22.5)(57.5,22.5)(55,22.5)(60,22.5)
\psbezier(60,22.5)(65,22.5)(65,18.75)(65,15)
}
\rput(82.5,5){}
\rput{0}(140,15){\psellipse[](0,0)(5,-5)}
\rput(120,15){$\scriptstyle 2s-1$}
\rput(140,15){$\scriptstyle 2s$}
\pscustom[]{\psbezier(90,35)(97.5,35)(117.5,35)(130,35)
\psbezier(130,35)(142.5,35)(145,18.75)(145,15)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(145,15)(145,5)(140,5)(130,5)
\psbezier[linestyle=dashed,dash=1 1](115,15)(115,5)(120,5)(130,5)
\rput[t](131.25,3.75){$\rho_{i,s}$}
\pscustom[]{\psbezier(10,15)(10,22.5)(16.25,35)(25,35)
\psbezier(25,35)(33.75,35)(85,35)(90,35)
}
\pscustom[]{\psbezier(72.5,30)(78.75,30)(100,30)(107.5,30)
\psbezier(107.5,30)(115,30)(115,18.75)(115,15)
}
\pscustom[]{\psbezier(10,15)(11.25,22.5)(17.5,30)(25,30)
\psbezier(25,30)(32.5,30)(68.75,30)(72.5,30)
}
\rput[t](10,12.5){$x_i$}
\psline[linestyle=dotted](97.5,15)(112.5,15)
\end{pspicture}


==> GFX/tore-X2b.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sat Sep 03 14:54:38 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="145" y-min="2.5" y-max="32.5" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2t-1$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(130,2.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_{j,t}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(140,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2t$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(40,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<ellipse p1="(115,20)" p2="(125,20)" p3="(125,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(65,20)" p2="(75,20)" p3="(75,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(85,20)" p2="(95,20)" p3="(95,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,15);(0,15);(10,15);(10,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,15);(20,15);(30,15);(30,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,15);(40,15);(50,15);(50,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(55,15);(55,15);(62.5,15);(62.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(10,15);(10,22.5);(28.75,25);(37.5,25);(46.25,25);(62.5,25);
%	(70,25)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(70,25);(77.5,25);(78.75,25);(85,25);(91.25,25);(95,18.75);
%	(95,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(95,15);(95,5);(90,5);(80,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(65,15);(65,5);(70,5);(80,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(10,15);(11.25,22.5);(32.5,22.5);(37.5,22.5);(42.5,22.5);(45,22.5);
%	(50,22.5)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(50,22.5);(57.5,22.5);(55,22.5);(60,22.5);(65,22.5);(65,18.75);
%	(65,15)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(82.5,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<ellipse p1="(135,20)" p2="(145,20)" p3="(145,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s-1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s$
%</text>
%<multicurve points="(112.5,32.5);(120,32.5);(120,32.5);(132.5,32.5);(145,32.5);(145,18.75);
%	(145,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(145,15);(145,5);(140,5);(130,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(115,15);(115,5);(120,5);(130,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(80,2.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_{i,s}$
%</text>
%<multicurve points="(2.5,15);(2.5,32.5);(2.5,32.5);(55,32.5);(107.5,32.5);(102.5,32.5);
%	(112.5,32.5)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(10,5);(2.5,5);(2.5,5);(2.5,15);(2.5,25);(0,30);
%	(55,30);(110,30);(115,18.75);(115,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,15);(40,20);(17.5,20);(17.5,15);(17.5,10);(17.5,5);
%	(10,5)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(10,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_i$
%</text>
%<multicurve points="(97.5,15);(97.5,15);(112.5,15);(112.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(145,32.5)
\rput(120,15){$\scriptstyle 2t-1$}
\rput[t](130,2.5){$z_{j,t}$}
\rput(140,15){$\scriptstyle 2t$}
\rput[t](40,12.5){$x_j$}
\rput{0}(120,15){\psellipse[](0,0)(5,-5)}
\rput{0}(70,15){\psellipse[](0,0)(5,-5)}
\rput{0}(90,15){\psellipse[](0,0)(5,-5)}
\psdots[](0,15)
(10,15)
\psdots[](20,15)
(30,15)
\psdots[](40,15)
(50,15)
\psline[linestyle=dotted](55,15)(62.5,15)
\pscustom[]{\psbezier(10,15)(10,22.5)(28.75,25)(37.5,25)
\psbezier(37.5,25)(46.25,25)(62.5,25)(70,25)
}
\pscustom[]{\psbezier(70,25)(77.5,25)(78.75,25)(85,25)
\psbezier(85,25)(91.25,25)(95,18.75)(95,15)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(95,15)(95,5)(90,5)(80,5)
\psbezier[linestyle=dashed,dash=1 1](65,15)(65,5)(70,5)(80,5)
\pscustom[]{\psbezier(10,15)(11.25,22.5)(32.5,22.5)(37.5,22.5)
\psbezier(37.5,22.5)(42.5,22.5)(45,22.5)(50,22.5)
}
\pscustom[]{\psbezier(50,22.5)(57.5,22.5)(55,22.5)(60,22.5)
\psbezier(60,22.5)(65,22.5)(65,18.75)(65,15)
}
\rput(82.5,5){}
\rput{0}(140,15){\psellipse[](0,0)(5,-5)}
\rput(70,15){$\scriptstyle 2s-1$}
\rput(90,15){$\scriptstyle 2s$}
\pscustom[]{\psbezier(112.5,32.5)(120,32.5)(120,32.5)(132.5,32.5)
\psbezier(132.5,32.5)(145,32.5)(145,18.75)(145,15)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(145,15)(145,5)(140,5)(130,5)
\psbezier[linestyle=dashed,dash=1 1](115,15)(115,5)(120,5)(130,5)
\rput[t](80,2.5){$z_{i,s}$}
\pscustom[]{\psbezier(2.5,15)(2.5,32.5)(2.5,32.5)(55,32.5)
\psbezier(55,32.5)(107.5,32.5)(102.5,32.5)(112.5,32.5)
}
\pscustom[]{\psbezier(10,5)(2.5,5)(2.5,5)(2.5,15)
\psbezier(2.5,15)(2.5,25)(0,30)(55,30)
\psbezier(55,30)(110,30)(115,18.75)(115,15)
}
\pscustom[]{\psbezier(40,15)(40,20)(17.5,20)(17.5,15)
\psbezier(17.5,15)(17.5,10)(17.5,5)(10,5)
}
\rput[t](10,12.5){$x_i$}
\psline[linestyle=dotted](97.5,15)(112.5,15)
\end{pspicture}


==> GFX/tore-X2c-incomplet.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Mon Sep 05 11:31:45 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="122.5" y-min="0" y-max="28.75" auto-bounding="true">
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(40,8.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<ellipse p1="(70,16.25)" p2="(80,16.25)" p3="(80,6.25)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(100,16.25)" p2="(110,16.25)" p3="(110,6.25)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,11.25);(0,11.25);(10,11.25);(10,11.25)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,11.25);(20,11.25);(30,11.25);(30,11.25)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,11.25);(40,11.25);(50,11.25);(50,11.25)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(55,11.25);(55,11.25);(60,11.25);(60,11.25)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(10,11.25);(11.25,18.75);(32.5,22.5);(32.5,11.25);(32.5,0);(36.25,0);
%	(40,0);(43.75,0);(47.5,0);(47.5,11.25)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(82.5,1.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(75,3.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s-1$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(105,3.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s$
%</text>
%<multicurve points="(100,11.25);(100,6.25);(95,5);(90,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(80,11.25);(80,5);(85,5);(90,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(40,11.25);(40,26.25);(46.25,25);(66.25,25)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(10,8.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_i$
%</text>
%<multicurve points="(113.75,11.25);(113.75,11.25);(122.5,11.25);(122.5,11.25)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(66.25,11.25);(66.25,11.25);(63.75,11.25);(63.75,11.25)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(70,11.25);(70,11.25);(66.25,11.25);(66.25,11.25)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(86.25,11.25);(86.25,11.25);(82.5,11.25);(82.5,11.25)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(82.5,11.25);(82.5,11.25);(80,11.25);(80,11.25)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(66.25,25);(82.5,25);(86.25,25);(86.25,16.25)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(86.25,16.25);(86.25,16.25);(86.25,11.25);(86.25,11.25)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="left" anchor-point="(101.25,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\alpha_2$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(65,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\alpha_1$
%</text>
%<text text-vert-align="bottom" text-hor-align="center-h" anchor-point="(82.5,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$f_1$
%</text>
%<multicurve points="(40,11.25);(40,28.75);(40,28.75);(82.5,28.75)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(82.5,28.75);(98.75,28.75);(100,27.5);(100,17.5)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(100,17.5);(100,17.5);(100,11.25);(100,11.25)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(66.25,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$f_1$
%</text>
%<multicurve points="(47.5,11.25);(47.5,22.5);(56.25,20);(66.25,20)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(66.25,20);(68.75,20);(70,20);(70,11.25)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(56.25,16.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\alpha_2$
%</text>
%<multicurve points="(47.5,11.25);(47.5,16.25);(50,17.5);(58.75,17.5)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<multicurve points="(58.75,17.5);(61.25,17.5);(63.75,17.5);(63.75,11.25)"
%	
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(122.5,28.75)
\rput[t](40,8.75){$x_j$}
\rput{0}(75,11.25){\psellipse[](0,0)(5,-5)}
\rput{0}(105,11.25){\psellipse[](0,0)(5,-5)}
\psdots[](0,11.25)
(10,11.25)
\psdots[](20,11.25)
(30,11.25)
\psdots[](40,11.25)
(50,11.25)
\psline[linestyle=dotted](55,11.25)(60,11.25)
\pscustom[]{\psbezier(10,11.25)(11.25,18.75)(32.5,22.5)(32.5,11.25)
\psbezier(32.5,11.25)(32.5,0)(36.25,0)(40,0)
\psbezier(40,0)(43.75,0)(47.5,0)(47.5,11.25)
}
\rput[t](82.5,1.25){}
\rput[t](75,3.75){$\scriptstyle 2s-1$}
\rput[t](105,3.75){$\scriptstyle 2s$}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(100,11.25)(100,6.25)(95,5)(90,5)
\psbezier[linestyle=dashed,dash=1 1](80,11.25)(80,5)(85,5)(90,5)
\psbezier{->}(40,11.25)(40,26.25)(46.25,25)(66.25,25)
\rput[t](10,8.75){$x_i$}
\psline[linestyle=dotted](113.75,11.25)(122.5,11.25)
\psline(66.25,11.25)(63.75,11.25)
\psline{->}(70,11.25)(66.25,11.25)
\psline{->}(86.25,11.25)(82.5,11.25)
\psline(82.5,11.25)(80,11.25)
\psbezier(66.25,25)(82.5,25)(86.25,25)(86.25,16.25)
\psline(86.25,16.25)(86.25,11.25)
\rput[l](101.25,22.5){$\alpha_2$}
\rput(65,22.5){$\alpha_1$}
\rput[b](82.5,12.5){$f_1$}
\psbezier(40,11.25)(40,28.75)(40,28.75)(82.5,28.75)
\psbezier{->}(82.5,28.75)(98.75,28.75)(100,27.5)(100,17.5)
\psline(100,17.5)(100,11.25)
\rput[t](66.25,10){$f_1$}
\psbezier{->}(47.5,11.25)(47.5,22.5)(56.25,20)(66.25,20)
\psbezier(66.25,20)(68.75,20)(70,20)(70,11.25)
\rput[t](56.25,16.25){$\alpha_2$}
\psbezier{->}(47.5,11.25)(47.5,16.25)(50,17.5)(58.75,17.5)
\psbezier(58.75,17.5)(61.25,17.5)(63.75,17.5)(63.75,11.25)
\end{pspicture}


==> GFX/tore-X2c.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sat Sep 03 14:52:12 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="0" y-max="35" auto-bounding="true">
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(40,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<ellipse p1="(68.75,21.25)" p2="(81.25,21.25)" p3="(81.25,8.75)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(100,20)" p2="(112.5,20)" p3="(112.5,7.5)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,15);(0,15);(10,15);(10,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,15);(20,15);(30,15);(30,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(40,15);(40,15);(50,15);(50,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(55,15);(55,15);(62.5,15);(62.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(10,15);(10,22.5);(15,35);(23.75,35);(32.5,35);(52.5,35);
%	(65,35)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(65,35);(72.5,35);(67.5,35);(90,35);(112.5,35);(112.5,22.5);
%	(112.5,13.75)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(112.5,13.75);(112.5,2.5);(106.25,2.5);(90,2.5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(68.75,15);(68.75,2.5);(68.75,2.5);(90,2.5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(10,15);(11.25,22.5);(32.5,26.25);(32.5,15);(32.5,3.75);(36.25,3.75);
%	(40,3.75);(43.75,3.75);(47.5,3.75);(47.5,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(47.5,15);(47.5,22.5);(51.25,22.5);(56.25,22.5);(61.25,22.5);(68.75,22.5);
%	(68.75,15)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(82.5,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(75,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s-1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(106.25,13.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2s$
%</text>
%<multicurve points="(40,15);(40,30);(40,30);(52.5,30);(65,30);(80,30);
%	(90,30);(100,30);(100,18.75);(100,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(100,13.75);(100,8.75);(95,8.75);(90,8.75)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(81.25,15);(81.25,8.75);(86.25,8.75);(91.25,8.75)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(91.25,0)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_{i,s}$
%</text>
%<multicurve points="(40,15);(40,23.75);(58.75,25);(60,25);(61.25,25);(81.25,25);
%	(81.25,15)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(10,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_i$
%</text>
%<multicurve points="(115,13.75);(115,13.75);(130,13.75);(130,13.75)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,35)
\rput[t](40,12.5){$x_j$}
\rput{0}(75,15){\psellipse[](0,0)(6.25,-6.25)}
\rput{0}(106.25,13.75){\psellipse[](0,0)(6.25,-6.25)}
\psdots[](0,15)
(10,15)
\psdots[](20,15)
(30,15)
\psdots[](40,15)
(50,15)
\psline[linestyle=dotted](55,15)(62.5,15)
\pscustom[]{\psbezier(10,15)(10,22.5)(15,35)(23.75,35)
\psbezier(23.75,35)(32.5,35)(52.5,35)(65,35)
}
\pscustom[]{\psbezier(65,35)(72.5,35)(67.5,35)(90,35)
\psbezier(90,35)(112.5,35)(112.5,22.5)(112.5,13.75)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(112.5,13.75)(112.5,2.5)(106.25,2.5)(90,2.5)
\psbezier[linestyle=dashed,dash=1 1](68.75,15)(68.75,2.5)(68.75,2.5)(90,2.5)
\pscustom[]{\psbezier(10,15)(11.25,22.5)(32.5,26.25)(32.5,15)
\psbezier(32.5,15)(32.5,3.75)(36.25,3.75)(40,3.75)
\psbezier(40,3.75)(43.75,3.75)(47.5,3.75)(47.5,15)
}
\pscustom[]{\psbezier(47.5,15)(47.5,22.5)(51.25,22.5)(56.25,22.5)
\psbezier(56.25,22.5)(61.25,22.5)(68.75,22.5)(68.75,15)
}
\rput(82.5,5){}
\rput(75,15){$\scriptstyle 2s-1$}
\rput(106.25,13.75){$\scriptstyle 2s$}
\pscustom[]{\psbezier(40,15)(40,30)(40,30)(52.5,30)
\psbezier(52.5,30)(65,30)(80,30)(90,30)
\psbezier(90,30)(100,30)(100,18.75)(100,15)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(100,13.75)(100,8.75)(95,8.75)(90,8.75)
\psbezier[linestyle=dashed,dash=1 1](81.25,15)(81.25,8.75)(86.25,8.75)(91.25,8.75)
\rput[t](91.25,0){$z_{i,s}$}
\pscustom[]{\psbezier(40,15)(40,23.75)(58.75,25)(60,25)
\psbezier(60,25)(61.25,25)(81.25,25)(81.25,15)
}
\rput[t](10,12.5){$x_i$}
\psline[linestyle=dotted](115,13.75)(130,13.75)
\end{pspicture}


==> GFX/tore-X2c2.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sat Sep 03 14:03:20 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="105" y-min="0" y-max="40" auto-bounding="true">
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(45,17.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<ellipse p1="(73.75,26.25)" p2="(86.25,26.25)" p3="(86.25,13.75)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(5,20);(5,20);(15,20);(15,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(25,20);(25,20);(35,20);(35,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(45,20);(45,20);(55,20);(55,20)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(60,20);(60,20);(67.5,20);(67.5,20)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(25,20);(20,27.5);(20,22.5);(12.5,22.5);(5,22.5);(5,27.5);
%	(0,20)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(0,20);(0,8.75);(15,7.5);(35,7.5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(73.75,20);(73.75,7.5);(55,7.5);(35,7.5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(25,20);(25,27.5);(37.5,27.5);(37.5,20);(37.5,12.5);(40,10);
%	(45,10);(50,10);(52.5,12.5);(52.5,20)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(52.5,20);(52.5,27.5);(56.25,27.5);(61.25,27.5);(66.25,27.5);(73.75,27.5);
%	(73.75,20)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(87.5,10)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(80,20)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2g-1$
%</text>
%<multicurve points="(45,20);(45,32.5);(50,32.5);(57.5,32.5);(65,32.5);(75,32.5);
%	(90,32.5);(105,32.5);(105,23.75);(105,20)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(105,20);(105,15);(100,13.75);(95,13.75)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(86.25,20);(86.25,13.75);(91.25,13.75);(96.25,13.75)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(33.75,6.25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_{i,g}$
%</text>
%<multicurve points="(45,20);(45,28.75);(57.5,30);(65,30);(72.5,30);(86.25,28.75);
%	(86.25,20)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(25,17.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_i$
%</text>
%<parallelogram p1="(0,40)" p2="(105,40)" p3="(105,0)"
%	
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(105,40)
\rput[t](45,17.5){$x_j$}
\rput{0}(80,20){\psellipse[](0,0)(6.25,-6.25)}
\psdots[](5,20)
(15,20)
\psdots[](25,20)
(35,20)
\psdots[](45,20)
(55,20)
\psline[linestyle=dotted](60,20)(67.5,20)
\pscustom[]{\psbezier(25,20)(20,27.5)(20,22.5)(12.5,22.5)
\psbezier(12.5,22.5)(5,22.5)(5,27.5)(0,20)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(0,20)(0,8.75)(15,7.5)(35,7.5)
\psbezier[linestyle=dashed,dash=1 1](73.75,20)(73.75,7.5)(55,7.5)(35,7.5)
\pscustom[]{\psbezier(25,20)(25,27.5)(37.5,27.5)(37.5,20)
\psbezier(37.5,20)(37.5,12.5)(40,10)(45,10)
\psbezier(45,10)(50,10)(52.5,12.5)(52.5,20)
}
\pscustom[]{\psbezier(52.5,20)(52.5,27.5)(56.25,27.5)(61.25,27.5)
\psbezier(61.25,27.5)(66.25,27.5)(73.75,27.5)(73.75,20)
}
\rput(87.5,10){}
\rput(80,20){$\scriptstyle 2g-1$}
\pscustom[]{\psbezier(45,20)(45,32.5)(50,32.5)(57.5,32.5)
\psbezier(57.5,32.5)(65,32.5)(75,32.5)(90,32.5)
\psbezier(90,32.5)(105,32.5)(105,23.75)(105,20)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(105,20)(105,15)(100,13.75)(95,13.75)
\psbezier[linestyle=dashed,dash=1 1](86.25,20)(86.25,13.75)(91.25,13.75)(96.25,13.75)
\rput[t](33.75,6.25){$z_{i,g}$}
\pscustom[]{\psbezier(45,20)(45,28.75)(57.5,30)(65,30)
\psbezier(65,30)(72.5,30)(86.25,28.75)(86.25,20)
}
\rput[t](25,17.5){$x_i$}
\pspolygon[](0,40)(105,40)(105,0)(0,0)
\end{pspicture}


==> GFX/tore-rho.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sat Sep 10 16:21:27 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="102.5" y-min="3.75" y-max="30" auto-bounding="true">
%<text text-vert-align="bottom" text-hor-align="center-h" anchor-point="(38.75,22.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$y_{r,u}^-$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(68.75,28.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$y_{r,u}^+$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2u-1$
%</text>
%<text text-vert-align="top" text-hor-align="center-h" anchor-point="(80,3.75)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$z_{r,u}$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2u$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(27.5,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_r$
%</text>
%<ellipse p1="(45,20)" p2="(55,20)" p3="(55,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(65,20)" p2="(75,20)" p3="(75,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(85,20)" p2="(95,20)" p3="(95,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(5,15);(5,15);(12.5,15);(12.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,15);(20,15);(27.5,15);(27.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(35,15);(35,15);(42.5,15);(42.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(57.5,15);(57.5,15);(62.5,15);(62.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(50,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$1$
%</text>
%<multicurve points="(27.5,15);(27.5,22.5);(27.5,30);(36.25,30);(45,30);(65,30);
%	(70,30)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" />
%<multicurve points="(97.5,15);(97.5,15);(102.5,15);(102.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(70,30);(77.5,30);(81.25,30);(87.5,30);(93.75,30);(95,18.75);
%	(95,15)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(95,15);(95,5);(90,5);(80,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 right-arrow="reverse-head" arrow-global-scale-width="1.5" />
%<multicurve points="(65,15);(65,5);(70,5);(80,5)"
%	 stroke-style="dashed" stroke-dasharray="1;1"
%	 fill-style="none"
%	 />
%<multicurve points="(27.5,15);(28.75,22.5);(31.25,21.25);(32.5,21.25);(33.75,21.25);(40,21.25);
%	(43.75,21.25)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="1.5" />
%<multicurve points="(43.75,21.25);(51.25,21.25);(58.75,21.25);(61.25,21.25);(63.75,21.25);(65,18.75);
%	(65,15)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(82.5,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%
%</text>
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(102.5,30)
\rput[b](38.75,22.5){$y_{r,u}^-$}
\rput[t](68.75,28.75){$y_{r,u}^+$}
\rput(70,15){$\scriptstyle 2u-1$}
\rput[t](80,3.75){$z_{r,u}$}
\rput(90,15){$\scriptstyle 2u$}
\rput(27.5,12.5){$x_r$}
\rput{0}(50,15){\psellipse[](0,0)(5,-5)}
\rput{0}(70,15){\psellipse[](0,0)(5,-5)}
\rput{0}(90,15){\psellipse[](0,0)(5,-5)}
\psdots[](5,15)
(12.5,15)
\psdots[](20,15)
(27.5,15)
\psdots[](35,15)
(42.5,15)
\psline[linestyle=dotted](57.5,15)(62.5,15)
\rput(50,15){$1$}
\pscustom[arrowscale=1.5 1]{\psbezier{-}(27.5,15)(27.5,22.5)(27.5,30)(36.25,30)
\psbezier{->}(36.25,30)(45,30)(65,30)(70,30)
}
\psline[linestyle=dotted](97.5,15)(102.5,15)
\pscustom[]{\psbezier(70,30)(77.5,30)(81.25,30)(87.5,30)
\psbezier(87.5,30)(93.75,30)(95,18.75)(95,15)
}
\psbezier[linestyle=dashed,dash=1 1,arrowscale=1.5 1]{-<}(95,15)(95,5)(90,5)(80,5)
\psbezier[linestyle=dashed,dash=1 1](65,15)(65,5)(70,5)(80,5)
\pscustom[arrowscale=1.5 1]{\psbezier{-}(27.5,15)(28.75,22.5)(31.25,21.25)(32.5,21.25)
\psbezier{->}(32.5,21.25)(33.75,21.25)(40,21.25)(43.75,21.25)
}
\pscustom[]{\psbezier(43.75,21.25)(51.25,21.25)(58.75,21.25)(61.25,21.25)
\psbezier(61.25,21.25)(63.75,21.25)(65,18.75)(65,15)
}
\rput(82.5,5){}
\end{pspicture}


==> GFX/tore-sigma-g.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sun Sep 11 19:14:14 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="0" y-max="32.5" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2g-1$
%</text>
%<multicurve points="(98.75,15);(98.75,15);(113.75,15);(113.75,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(5,15);(5,15);(12.5,15);(12.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,15);(20,15);(27.5,15);(27.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(35,15);(35,15);(42.5,15);(42.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(57.5,15);(57.5,15);(62.5,15);(62.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(50,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle u-1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$u$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(27.5,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<text text-vert-align="baseline" text-hor-align="center-h" anchor-point="(70,5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\sigma_{j,2g}$
%</text>
%<multicurve points="(60,2.5);(42.5,2.5);(37.5,2.5);(20,2.5);(2.5,2.5);(2.5,2.5);
%	(2.5,15);(2.5,27.5);(2.5,27.5);(17.5,27.5)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<parallelogram p1="(0,30)" p2="(130,30)" p3="(130,0)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(95,32.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$D_{2g}$
%</text>
%<multicurve points="(92.5,30);(92.5,30);(102.5,30);(102.5,30)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" />
%<ellipse p1="(45,20)" p2="(55,20)" p3="(55,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(65,20)" p2="(75,20)" p3="(75,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(85,20)" p2="(95,20)" p3="(95,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(115,20)" p2="(125,20)" p3="(125,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(27.5,15);(27.5,27.5);(27.5,27.5);(32.5,27.5);(37.5,27.5);(92.5,27.5);
%	(110,27.5);(127.5,27.5);(127.5,27.5);(127.5,15)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<multicurve points="(127.5,15);(127.5,2.5);(127.5,2.5);(110,2.5);(92.5,2.5);(67.5,2.5);
%	(60,2.5)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" arrow-global-scale-length="2" />
%<multicurve points="(17.5,27.5);(27.5,27.5);(27.5,27.5);(27.5,15)"
%	
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,32.5)
\rput(120,15){$\scriptstyle 2g-1$}
\psline[linestyle=dotted](98.75,15)(113.75,15)
\psdots[](5,15)
(12.5,15)
\psdots[](20,15)
(27.5,15)
\psdots[](35,15)
(42.5,15)
\psline[linestyle=dotted](57.5,15)(62.5,15)
\rput(50,15){$1$}
\rput(70,15){$\scriptstyle u-1$}
\rput(90,15){$u$}
\rput(27.5,12.5){$x_j$}
\rput[B](70,5){$\sigma_{j,2g}$}
\pscustom[arrowscale=2 2]{\psbezier{-}(60,2.5)(42.5,2.5)(37.5,2.5)(20,2.5)
\psbezier(20,2.5)(2.5,2.5)(2.5,2.5)(2.5,15)
\psbezier{->}(2.5,15)(2.5,27.5)(2.5,27.5)(17.5,27.5)
}
\pspolygon[](0,30)(130,30)(130,0)(0,0)
\rput(95,32.5){$D_{2g}$}
\psline[arrowscale=2 1]{->}(92.5,30)(102.5,30)
\rput{0}(50,15){\psellipse[](0,0)(5,-5)}
\rput{0}(70,15){\psellipse[](0,0)(5,-5)}
\rput{0}(90,15){\psellipse[](0,0)(5,-5)}
\rput{0}(120,15){\psellipse[](0,0)(5,-5)}
\pscustom[arrowscale=2 2]{\psbezier{-}(27.5,15)(27.5,27.5)(27.5,27.5)(32.5,27.5)
\psbezier(32.5,27.5)(37.5,27.5)(92.5,27.5)(110,27.5)
\psbezier{->}(110,27.5)(127.5,27.5)(127.5,27.5)(127.5,15)
}
\pscustom[arrowscale=2 2]{\psbezier{-}(127.5,15)(127.5,2.5)(127.5,2.5)(110,2.5)
\psbezier{->}(110,2.5)(92.5,2.5)(67.5,2.5)(60,2.5)
}
\psbezier(17.5,27.5)(27.5,27.5)(27.5,27.5)(27.5,15)
\end{pspicture}


==> GFX/tore-sigma.tex <==
%%Created by jPicEdt 1.4pre4: mixed JPIC-XML/LaTeX format
%%Sun Sep 11 19:15:05 CEST 2005
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="0" y-max="32.5" auto-bounding="true">
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(120,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle 2g-1$
%</text>
%<multicurve points="(98.75,15);(98.75,15);(113.75,15);(113.75,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<multicurve points="(5,15);(5,15);(12.5,15);(12.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(20,15);(20,15);(27.5,15);(27.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(35,15);(35,15);(42.5,15);(42.5,15)"
%	 polydots-style="polydots-disk" polydots-size-minimum="0.7" polydots-size-linewidth-scale="2.5" polydots-angle="0"
%	 polydots-scale-h="1" polydots-scale-v="1" polydots-superimpose="false"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(57.5,15);(57.5,15);(62.5,15);(62.5,15)"
%	 stroke-style="dotted"
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(50,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(70,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\scriptstyle u-1$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(90,15)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$u$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(27.5,12.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$x_j$
%</text>
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(52.5,25)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$\sigma_{j,u}$
%</text>
%<multicurve points="(27.5,15);(27.5,22.5);(27.5,22.5);(35,22.5);(42.5,22.5);(85,22.5);
%	(90,22.5);(95,22.5);(97.5,20);(97.5,15);(97.5,10);(95,7.5);
%	(90,7.5)"
%	
%	 fill-style="none"
%	 />
%<multicurve points="(90,22.5);(85,22.5);(82.5,20);(82.5,15);(82.5,10);(85,7.5);
%	(90,7.5)"
%	
%	 fill-style="none"
%	 right-arrow="head" />
%<parallelogram p1="(0,30)" p2="(130,30)" p3="(130,0)"
%	
%	 fill-style="none"
%	 />
%<text text-vert-align="center-v" text-hor-align="center-h" anchor-point="(10,32.5)" text-frame="noframe"
%	
%	 fill-style="none"
%	 >
%$D_{2g}$
%</text>
%<multicurve points="(5,30);(5,30);(15,30);(15,30)"
%	
%	 fill-style="none"
%	 right-arrow="head" arrow-global-scale-width="2" />
%<ellipse p1="(45,20)" p2="(55,20)" p3="(55,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(65,20)" p2="(75,20)" p3="(75,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(85,20)" p2="(95,20)" p3="(95,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%<ellipse p1="(115,20)" p2="(125,20)" p3="(125,10)" angle-start="0" angle-end="0" closure="open"
%	
%	 fill-style="none"
%	 />
%</jpic>
%%End JPIC-XML
%PsTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
\psset{xunit=1mm,yunit=1mm,runit=1mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,32.5)
\rput(120,15){$\scriptstyle 2g-1$}
\psline[linestyle=dotted](98.75,15)(113.75,15)
\psdots[](5,15)
(12.5,15)
\psdots[](20,15)
(27.5,15)
\psdots[](35,15)
(42.5,15)
\psline[linestyle=dotted](57.5,15)(62.5,15)
\rput(50,15){$1$}
\rput(70,15){$\scriptstyle u-1$}
\rput(90,15){$u$}
\rput(27.5,12.5){$x_j$}
\rput(52.5,25){$\sigma_{j,u}$}
\pscustom[]{\psbezier(27.5,15)(27.5,22.5)(27.5,22.5)(35,22.5)
\psbezier(35,22.5)(42.5,22.5)(85,22.5)(90,22.5)
\psbezier(90,22.5)(95,22.5)(97.5,20)(97.5,15)
\psbezier(97.5,15)(97.5,10)(95,7.5)(90,7.5)
}
\pscustom[]{\psbezier{-}(90,22.5)(85,22.5)(82.5,20)(82.5,15)
\psbezier{->}(82.5,15)(82.5,10)(85,7.5)(90,7.5)
}
\pspolygon[](0,30)(130,30)(130,0)(0,0)
\rput(10,32.5){$D_{2g}$}
\psline[arrowscale=2 1]{->}(5,30)(15,30)
\rput{0}(50,15){\psellipse[](0,0)(5,-5)}
\rput{0}(70,15){\psellipse[](0,0)(5,-5)}
\rput{0}(90,15){\psellipse[](0,0)(5,-5)}
\rput{0}(120,15){\psellipse[](0,0)(5,-5)}
\end{pspicture}

